COCOA: CBT-based Conversational Counseling Agent using Memory Specialized in Cognitive Distortions and Dynamic Prompt

The demand for conversational agents that provide mental health care is consistently increasing. In this work, we develop a psychological counseling agent, referred to as CoCoA, that applies Cognitive Behavioral Therapy (CBT) techniques to identify and address cognitive distortions inherent in the client's statements. Specifically, we construct a memory system to efficiently manage information necessary for counseling while extracting high-level insights about the client from their utterances. Additionally, to ensure that the counseling agent generates appropriate responses, we introduce dynamic prompting to flexibly apply CBT techniques and facilitate the appropriate retrieval of information. We conducted dialogues between CoCoA and characters from Character.ai, creating a dataset for evaluation. Then, we asked GPT to evaluate the constructed counseling dataset, and our model demonstrated a statistically significant difference from other models.

==> 3_method_new.tex <==
\section{LLM as a Counselor : CoCoA}
\subsection{Overview}
In this section, we present the Counselor Agent, referred to as \textbf{CoCoA}. As shown in Figure 1, our framework consists of two components: 1) memory management, and 2) prompt composition. When constructing prompts, the required information is retrieved from the memory and used accordingly. The constructed prompt is served as input to the LLM, denoted as $\mathcal{F}$.

\begin{figure*}
\begin{center}
%\includegraphics[width=0.8\linewidth]{figures/CoCoA agent.png}
\includegraphics[width=0.8\linewidth]{figures/cocoa3.png}

\end{center}
\caption{CoCoA agent architecture}
\label{fig:short}
\end{figure*}


\noindent\textbf{Memory Management}. The counselor stores the information gathered during counseling sessions in memory to provide appropriate responses. Each time client utterances are received, the system draws insights from them and stores insights in the basic memory. If any cognitive distortions are identified during the conversation, they are saved in the cognitive distortion memory.

\noindent\textbf{Prompt Composition}. 
We structure prompts into static $S$ and dynamic $D$ prompts. The static prompt remains unchanged as the conversation progresses, providing a consistent reference. On the other hand, the dynamic prompt is customized for each turn, retrieving knowledge from external sources to generate contextually relevant prompts that fit the current situation. This approach is adopted to flexibly apply Cognitive Behavioral Therapy (CBT) techniques and facilitate the appropriate retrieval of information required during the technique application.

\subsection{Memory Management}

The client information storage system has two components: \textit{Basic Memory} and \textit{Cognitive Distortion Memory}, referred to as \textit{CD Memory}. %Our research aims to provide long-term and multi-session counseling to our clients. To achieve that, it is imperative to store counseling records for each client. Moreover, 
To emulate a human counselor aiming to identify core beliefs embedded across multiple episodes and integrate them for cognitive distortion resolution, we manage and store the cognitive distortion memory from the the basic memory.


\textit{Basic Memory} stores the information obtained about the client during counseling sessions. When client utterances are received as input, the system extracts high-level insights from the client's expression. This information about the client is then stored in the basic memory. \textit{CD Memory} analyzes each utterance made by the client to identify any cognitive distortions. If a cognitive distortion is detected, the system saves the cognitive type, the utterance made, and a score on a Likert scale from 1 to 5, indicating the severity of the distortion.

% cd memory 구축한 후 cd to treat 정함
After constructing \textit{CD Memory}, the system proceeds to determine the cognitive distortion type that will be prioritized for treatment among the existing cognitive distortions. To determine which type of cognitive distortion to treat, the agent considers three main components: \textit{recency}, \textit{frequency}, and \textit{severity}, as inspired by the \citet{park2023generative}. \textit{Recency} assigns a higher score to the most recently mentioned cognitive distortion, using an exponential decay function over the number of utterances ago. \textit{Frequency} counts the occurrences of each cognitive distortion. \textit{Severity} is determined by the score from 1 to 5 on a Likert scale for each cognitive distortion stored in the CD memory.
The final score is calculated by normalizing the \textit{recency}, \textit{frequency}, and \textit{severity} scores to a value between 0 and 1, and then combining them using weighted coefficients. Thus the scoring function can be denoted as $
\textit{{S}} = \alpha_{\textit{recency}} \times \textit{{recency}} + \alpha_{\textit{frequency}} \times \textit{{frequency}} + \alpha_{\textit{severity}} \times \textit{{severity}}$.
The type of cognitive distortion that maximizes the score function among those present in the CD memory is adopted as Cognitive distortion type to treat, referred to as $cd^*$. 


\begin{equation}
cd^* = \underset{cd  \in CD}{\text{argmax}}  \textit{ S}(cd)
\end{equation}






% cognitive memory에서 관련 기억 retrieval하는 것 - 심리학에서의 Priming Effect, 진짜 인간처럼 어떤 말을 들었을 때, 그 말과 관련된 것들도 떠올리는 특징을 고려해서 메모리를 만들었다.

\subsection{Prompt Composition}
\subsubsection{Static Prompt}
The static prompt consists of a task description $T$, an explanation of the strategies of the ESC technique $ESC$, and the most recent utterances $U$. Thus, the static prompt can be denoted as $S = (T, ESC, U)$.

\subsubsection{Dynamic Prompt}
The Dynamic prompt is composed of three main processes: 1) determining the applicable CBT technique, 2) specifying the CBT stage to apply, and 3) generating responses based on these determinations.


\noindent\textbf{CBT Technique Determination} We present the algorithm for determining CBT Technique in Alg. 1. Based on the cognitive distortion type $CD$ determined in memory management, the system retrieves related information from both \textit{Basic Memory} and \textit{CD Memory}. In this process, we use the Contriever\citep{lei2023unsupervised} to retrieve memories by embedding memories and calculating the similarity between them. CBT technique to apply $Tech$ is selected based on the retrieved memories $M_r$, and then background information related to the chosen CBT technique is additionally retrieved for use in the next step of dynamic prompt.

% \begin{algorithm}
% \caption{ Determine CBT Technique}
% \textbf{Input:} \mathcal{F}, CD

% \textbf{Output:} Tech

% \medskip

% M_r \leftarrow Contriever(\textit{Basic Memory}, \textit{CD Memory}|CD)

% Tech \leftarrow \mathcal{F}(\cdot|M_r)

% \end{algorithm}

\noindent\textbf{CBT Stage Determination} In the subsequent step, the agent is tasked with selecting a specific stage $Stage$ from the various stages of the chosen CBT technique. First, information about the stages involved in the CBT technique, decided upon in the previous step, is retrieved. Subsequently, based on the CBT process log $Log$, which records the progress of CBT techniques used so far, and the determined CBT technique applied in the conversation, the next steps in the CBT process are determined. This process can be represented as: 

% \begin{algorithm}
% \caption{ Determine CBT Stage}
% \textbf{Input:} \mathcal{F}, Tech, Log

% \textbf{Output:} Stage

% \medskip

% CBT doc \leftarrow \mathcal{F}(\cdot|Tech)

% Stage \leftarrow \mathcal{F}(\cdot|CBT doc, Log)

% \end{algorithm}

\noindent\textbf{Response Generation} Based on the CBT technique and stage chosen in the preceding two steps, the agent retrieves an example of counselor's appropriate utterances $EX$ for the stage. The dynamic prompt, composed of these three pieces of information, is combined with the static prompt and served into LLM as an input, resulting in the generation of a response. This procedure can be illustrated as:
% $$ EX \sim \mathcal{F}(\cdot|Stage)$$
% $$D \sim \mathcal{F}(\cdot|EX, Stage, Tech) $$
% \begin{algorithm}
% \caption{ Generate Response}
% \textbf{Input:} \mathcal{F}, Tech, Stage

% \textbf{Output:} Response

% \medskip

% EX \leftarrow \mathcal{F}(\cdot|Stage)

% Response \leftarrow \mathcal{F}(\cdot|EX, Stage, Tech)

% \end{algorithm}



% \begin{algorithm}
% \caption{ CoCoA}
% \textbf{Input:} \mathcal{F}, \textit{Basic Memory}, \textit{CD Memory}

% \textbf{Output:} Response

% \medskip

% CD^* \leftarrow \underset{cd  \in CD}{\text{argmax}}  \textit{ S}(cd)

% M_r \leftarrow Contriever(\textit{Basic Memory}, \textit{CD Memory}|CD^*)

% Tech \leftarrow \mathcal{F}(\cdot|M_r)

% CBT doc \leftarrow \mathcal{F}(\cdot| Tech)

% Stage \leftarrow \mathcal{F}(\cdot| CBT doc, Log)

% EX \leftarrow \mathcal{F}(\cdot|Stage)

% Response \leftarrow \mathcal{F}(\cdot|EX, Stage, Tech)

% \end{algorithm}

% \makeatletter
% \algrenewcommand\ALG@beginalgorithmic{\footnotesize}
% \algrenewcommand\algorithmiccomment[2][\normalsize]{{#1\hfill\(\triangleright\) #2}}
% \makeatother

%\begin{algorithm}
%\caption{Memory Management}
%\begin{algorithmic}[0]
%\noindent \textbf{Input : } 
%\newline \hspace*{1em} $p_{i}$, \; Client's \textit{i-th} utterance;
%\newline \hspace*{1em} $f_{LLM}$, \; LLM Model;
%\newline \noindent \textbf{Output : } 
%\newline \hspace*{1em} $M_{B}$, \; Basic Memory;
%\newline \hspace*{1em} $M_{CD}$, \; CD Memory;
%\newline

%\newline $M_{B} \leftarrow$ Insight($p_{n}, ..., p_{n-k}$)
%\newline \textbf{if} $cd$ in ($p_{n}, ..., p_{n-k}$)  \; \textbf{then}
%\newline \hspace*{1em} $M_{CD}$ $\leftarrow$ ($cd$)
%\newline \textbf{endif}
%\newline \textbf{return} $M_{B}, M_{CD}$
%\end{algorithmic}
%\end{algorithm}






==> 4_exp.tex <==
\section{Experiments}
\subsection{Classification for Cognitive Distortion}

It is crucial to identify cognitive distortions inherent in the client’s expressions proactively to conduct counseling using the CBT techniques. Detecting the presence and types of cognitive distortions, which occur unconsciously in the client’s thought process, can be a challenging task. Therefore, we aim to evaluate the performance of the counseling agent by assessing its ability to effectively identify the existence and types of cognitive distortions.


\noindent\textbf{Dataset} 
We acquire 698 cognitive distortion data from Thinking Traps Dataset\cite{sharma2023cognitive} and 600 from Reframing Dataset\cite{sharma2023cognitive}. Each dataset consists of (1) utterances containing one or two sentences and (2) the corresponding cognitive distortion type.
%For the experiment, we utilized Thinking Traps dataset and Reframing dataset\cite{sharma2023cognitive} labeled with cognitive distortions based on utterances. Thinking Traps dataset consists of 698 instances, where utterances are connected to cognitive errors, including 14 types of cognitive errors, with "not distorted" being one of them. Reframing dataset comprises 600 instances, linking situations, thoughts about those situations, and cognitive errors embedded in those thoughts. It encompasses 15 types of cognitive errors, including "not distorted."
%This datasets were annotated by 15 mental health practitioners and clinical psychology graduate students with practical experience in cognitive reframing.

\noindent\textbf{Baselines} We performed experiments on each dataset using various prompts to analyze which prompting are most beneficial for detecting cognitive distortions.
We investigated how the separation of the step to identify the presence of cognitive errors affects performance. Additionally, we examined how performance varies based on the number of few shots provided when presenting few shots.



\noindent\textbf{Experimental Results} As shown in Table 1, prompting only with examples for cognitive distortions achieves the best performance. In cases where both description and examples were not provided, the classification accuracy performance was remarkably low at 11.46\%. A substantial improvements are observed on the method with description or examples in the prompt. Despite the enhanced performance, the accuracy remains relatively low, indicating persistent limitations.

\begin{table}[]
\centering
\begin{tabular}{ll}
\hline
\multicolumn{1}{c}{\textbf{Method}}  & \multicolumn{1}{c}{\textbf{Acc}} \\ \hline
\textit{w/o} description \& examples & 11.46                            \\ 
\textit{w/} description \& examples  & 33.38                            \\
\textit{w/} description             & 33.38                             \\
\textbf{\textit{w/} examples}       & \textbf{34.67}                   \\  \hline
\end{tabular}
\caption{Performance on the effect of prompting with description and examples}
\end{table}

\subsection{Response Generation Evaluation}
In order to evaluate how well \textbf{CoCoA} performs as a counselor, it is necessary to engage in the conversations between \textbf{CoCoA} and the interlocutor and compare its conversation dataset with those of other LLMs.
To meet this end, we facilitated conversations between the counselor agents and the interlocutor agent, who acts as a client, to generate counseling conversation datasets. Subsequently, we asked \texttt{GPT-3.5-turbo} to rate the constructed dataset with each of the five criteria using a scale of 0 to 6.

% 결론으로 빠져도 될 것 같습니다
%The collection of counseling datasets faces practical limitations due to privacy and ethical issues in actual data gathering. While creating a crowdsourced counseling dataset is possible, it incurs significant costs, and considering long and multi-session counseling poses challenges.

\subsubsection{Evaluation Dataset Construction} 
We opted to use a character.ai\footnote{https://beta.character.ai/} chatbot service to play the role of the client. Character.ai is a conversational agent service that allows you to have a conversation with simulacra created about famous people. We sampled 8 simulacra from character.ai and engaged in conversation with them. The chosen character can be verified in Appendix \ref{sec:appendixb}. We compare our models with three baselines: \texttt{GPT-3.5-turbo}, \texttt{LLAMA 7B}\cite{touvron2023llama} and \texttt{Vicuna 7B}\cite{zheng2023judging}.

\subsubsection{Evaluation Criteria}
The evaluation criteria consist of five elements which are derived from \cite{blackburn2001revised} and \cite{shao2023character}. Three of these elements are related to the validity, appropriateness, and accuracy of the CBT technique application, one is related to the execution of emotionally supportive dialogue, and the other one is about the stability of the model. Each element is rated on a scale of 0 to 6.
\begin{itemize}
    \item \textbf{CBT Validity}: The model's ability to choose the optimal technique based on valid reasoning, considering the targeted dysfunctional thoughts and the client's core issues.
    \item \textbf{CBT Appropriateness}: The model should maintain a cooperative attitude, focusing on enabling the client to explore their issues rather than engaging in argumentation or persuasion when using CBT techniques.
    \item \textbf{CBT Accuracy}: The model should use the selected CBT techniques accurately and proficiently.
    \item \textbf{ES Appropriateness}: The model should engage in conversation that remains within the context of the preceding dialogue or general common sense, offering appropriate empathy and comfort.
    \item \textbf{Stability}: The model should remain stable and consistent during relatively long conversations, even in the face of variations in incremental inputs.
    
\end{itemize}



\begin{figure*}
\begin{center}
\includegraphics[width=0.8\linewidth]{figures/evaluation.png}
\end{center}
\caption{Evaluation results}
\label{fig:evals}
\end{figure*}
\subsubsection{Evaluation Results}
Results are shown in Figure \ref{fig:evals}. We first calculate the average score for each criterion. Compared to Vicuna, our model scores higher in all criteria. It generally exhibits high performance on CBT Validity and Accuracy compared to other models. However, there are not a significant difference in ES Appropriateness or Stability.

To determine whether these differences are statistically significant, we use t-test. The results show no significant difference in the Stability, but there are significant differences in the other criteria.

In this paper, we mainly focus on counseling settings that utilize CBT techniques. The results prove the effectiveness of our proposed model, \textbf{CoCoa}.
%However, while this service adeptly reflects character traits, it may have limitations compared to real-world data. 





% As the conversational agent generates natural language, it is challenging to evaluate its performance using conventional evaluation metrics such as BLEU or ROUGE\cite{liu2023gpteval}. Due to this reason, prior studies conduct human evaluation, where human workers assign scores based on the given criteria. Additionally, some studies utilize Large Language Models(LLM) as evaluators\cite{liu2023chatcounselor}.


% To evaluate the performance of the counselor agent, it is necessary to have a deep understanding of CBT technique. Therefore, only a psychotherapist who is well-versed in CBT can provide a reliable assessment, which sets it apart from other conversational agents that can be evaluated by the public. To overcome this limitation, we used LLM evaluation to assess the conversations between the agents. To ensure the reliability of the LLM evaluation results, we also employed human evaluation for a subset of sampled data and compared it with the LLM evaluation results.

% We had LLMs rate the score of dialogues between the counselor and the client agents on a scale of 1 to 5 based on criteria such as fluency and appropriate use of counseling techniques. Additionally, we sampled the counseling dataset and had CBT technique experts evaluate the dataset based on the same evaluation criteria.

% \subsection{Experiment}
% We conducted two experiments to demonstrate the similarity between human evaluation and LLM evaluation results.
% First, we built a counseling dataset with varying parameters for the GPT model and evaluated it. The evaluation scores for the counseling dataset increased as the model's parameters increased. Second, we performed a correlation analysis between the scores for each criterion and he overall scores obtained from human evaluation and LLM evaluation. The Pearson correlation coefficient was 0.**, indicating a high similarity between human evaluation and LLM evaluation.

==> 5_results.tex <==

\section{Evaluation}

We evaluate our model to analyze the performance of counseling based on CBT. We compare our models with three baselines : ChatGPT, Alpaca 7B, and Vicuna 7B. We ask GPT-3.5 to rate the performance on the evaluation criteria. 

\subsection{Evaluation Criteria}
The evaluation criteria consist of four elements based on \cite{blackburn2001revised} : three related to the validity, appropriateness, and accuracy of CBT technique usage, and one related to conducting emotional supportive dialogue appropriately. Scores range from 0 to 6.
\begin{itemize}
    \item \textbf{CBT Validity}: The model's ability to choose the optimal technique based on valid reasoning, considering the targeted dysfunctional thoughts and the client's core issues.
    \item \textbf{CBT Appropriateness}: The model should maintain a cooperative attitude, focusing on enabling the client to explore their issues rather than engaging in argumentation or persuasion when using CBT techniques.
    \item \textbf{CBT Accuracy}: The model should use the selected CBT techniques accurately and proficiently.
    \item \textbf{ES Appropriateness}: The model should engage in conversation that remains within the context of the preceding dialogue or general common sense, offering appropriate empathy and comfort.
    \item \textbf{Stability}: The model should maintain a good performance over the long interaction.
\end{itemize}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/evaluation.png}
    \caption{Evaluation results}
    \label{fig:enter-label}
\end{figure}

\subsection{Evaluation Results}
Results are shown in \ref{fig:enter-label}. We first calculate the average score for each criterion. Compared to ChatGPT, our model scores higher in all criteria. To determine whether these differences are statistically significant, we use t-test. The results show no significant difference in the CBT appropriateness, but there are significant differences in the other criteria.


% % \input{tables/main_table}
% \subsection{Main Results}
% \paragraph{Comparison with Baselines.}

% % \input{tables/bio_table}
% The main results are shown in Table~\ref{tab:main_results}. (...)

% \paragraph{Error Type Analysis.}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=1\columnwidth]{figures/error_analysis.png}
%     \caption{Error analysis. (temporary figure)}
%     \label{fig:error_analysis} 
% \end{figure} 

% Error type analysis is shown in Figure~\ref{fig:error_analysis}. (...)

% \input{tables/ablation}
% \paragraph{Ablation study.}

% To see how components in our framework contributes to performance gain, we create multiple variants by removing each component individually. First, we remove evidence generation to show that contextualizing knowledge effectively enhances performance. As shown in the first row of Table~\ref{tab:ablation}, (...)

% 추출에 필요한 rationale을 LLM이 생성하게 해서 더 나은 결과가 나올 수 있도록 함
% As shown in Table~\ref{tab:ablation}, we witness that removing any component from our framework significantly degrades performance. This observation verifies the effectiveness of reasoning path and self-consistency.


% % \input{tables/example}

% \paragraph{Case study.} (...)


% \subsection{Generalization on Unseen Data}

% In this section, we observe if our framework is also feasible for real-world scenarios where collecting expert-annotated dataset may not be available in most practical cases.

% To further show the effectiveness of our framework even on unseen settings, we apply our \verifiner~on cross-inferred dataset, where models trained on source dataset are inferred on target dataset. Implementation details are in Appendix~\ref{sec:appendix}.

% As results are shown in Table~\ref{tab:cross_dataset_results}, we discover that our framework has generalization ability in unseen datasets without significant performance degradation, compared to LLM-based NER model. 

% \input{tables/cross_dataset}



% \clearpage

% \input{tables/goal}


==> 7_limit.tex <==
% \section{Limitation}
% 다른 task에도 적용
% KB의 특성에 따라 조금 달라질 수 있음 (?)
% llm 하나밖에 안쓴거?
% (...)
% \begin{itemize}
%     \item Only used ChatGPT for LLMㅈ
%     \item Application on other task
% \end{itemize}
% TEXT DUMP TEXT DUMP TEXT DUMP TEXT DUMP TEXT DUMP TEXT DUMP TEXT DUMP TEXT DUMP TEXT DUMP TEXT DUMP TEXT DUMP TEXT DUMP TEXT DUMP TEXT DUMP TEXT DUMP TEXT DUMP TEXT DUMP TEXT DUMP TEXT DUMP TEXT DUMP TEXT DUMP TEXT DUMP TEXT DUMP TEXT DUMP TEXT DUMP TEXT DUMP 

==> figure_latex/figure2.tex <==
% \begin{figure*}[ht]
%     \centering
%     \includegraphics[width=1\textwidth]{figures/figure2.pdf}
%     \caption{\textit{Top:} Verification-augmented NER. \textit{Bottom:} Overview of \verifiner. (work in progress)}
%     \label{fig:overview} ~
% \end{figure*} 

==> tables/ablation.tex <==
\begin{table}[h]
% \small
\centering
\resizebox{1.\columnwidth}{!}{
\begin{tabular}{llccc}
\toprule
 & &
  % \multicolumn{3}{c}{\textbf{BC5CDR}} &
  \multicolumn{3}{c}{\textbf{GENIA}} \\ 
  \cmidrule(l){3-5} 
  % \cmidrule(l){5-7} 
  
& &
  % P &
  % R &
  % F &
  P &
  R & 
  F \\ 
\toprule

% \textsc{\verifiner} ($n$=20) &- & - & - & \textbf{72.62} & 44.38 & 55.09 \\ 
% \textsc{GPT-NER} \\

\multirow{6}{*}{\textsc{GPT-NER}} & \hspace{0.1cm}+{\verifiner} ($n$=10) & 72.37 & \textbf{44.95} & \textbf{55.46} \\ 
&\hspace{0.1cm}+{\verifiner} ($n$=20) & \textbf{72.62} & 44.38 & 55.09 \\ 

&\hspace{0.3cm} w/o KB & 46.05 & 32.93 & 38.40 \\
&\hspace{0.3cm} w/o evidence & - & - & -  \\
&\hspace{0.3cm} w/o SC & 71.57 & 42.95 & 53.68 \\
&\hspace{0.3cm} w/o evidence, SC & 43.49 & 34.32 & 38.36 \\ \midrule

\multirow{5}{*}{\textsc{ConNER}} & \hspace{0.1cm}+{\verifiner} ($n$=10) & \textbf{79.07} & \textbf{91.82} & \textbf{84.97} \\ 

&\hspace{0.3cm} w/o KB & - & - & - \\
&\hspace{0.3cm} w/o evidence & - & - & -  \\
&\hspace{0.3cm} w/o SC & 77.63 & 86.14 & 81.66 \\
&\hspace{0.3cm} w/o evidence, SC & 52.70 & 91.09 & 66.77 \\
\bottomrule

\end{tabular}}
\caption{Ablation study results on GENIA prediction.}
\label{tab:ablation}
\end{table}





% \begin{table*}[h]
% % \small
% \centering
% % \resizebox{1.\columnwidth}{!}{
% \begin{tabular}{lcccccc}
% \toprule
%  &
%   % \multicolumn{3}{c}{\textbf{BC5CDR}} &
%   \multicolumn{3}{c}{\textsc{GPT-NER}} &
%   \multicolumn{3}{c}{\textsc{ConNER}} \\ 
%   \cmidrule(lr){2-4} 
%   \cmidrule(l){5-7} 
  
% % \textbf{Models} & 
% \textbf{} & 
%   P &
%   R &
%   F &
%   P &
%   R & 
%   F \\ 
% \toprule

% \hspace{0.1cm}+{\verifiner} ($n$=10) & 72.37 & \textbf{44.95} & \textbf{55.46} & \textbf{79.07} & \textbf{91.82} & \textbf{84.97}\\ 
% \hspace{0.1cm}+{\verifiner} ($n$=20) & \textbf{72.62} & 44.38 & 55.09 & - & - & -\\ 

% \hspace{0.3cm} w/o KB & 46.05 & 32.93 & 38.40 & - & - & - \\
% \hspace{0.3cm} w/o evidence & - & - & - & - & - & - \\
% \hspace{0.3cm} w/o SC & 71.57 & 42.95 & 53.68 & 77.63 & 86.14 & 81.66 \\
% \hspace{0.3cm} w/o evidence, SC & 43.49 & 34.32 & 38.36 & 52.70 & 91.09 & 66.77 \\ 
% \bottomrule

% \end{tabular}
% % }
% \caption{Ablation study results of GPT-NER and ConNER on GENIA prediction.}
% \label{tab:ablation}
% \end{table*}

==> tables/bio_table.tex <==
\begin{table*}[ht]
\small
\centering
\begin{tabular}{lcccccc}
\toprule
 &
  \multicolumn{3}{c}{\textbf{BC5CDR}} &
  \multicolumn{3}{c}{\textbf{GENIA}} \\ 
  \cmidrule(lr){2-4} \cmidrule(l){5-7}
  
% \textbf{Models} & 
\textbf{} & 
  Precision &
  Recall &
  F1 &
  Precision &
  Recall &
  F1 \\ 
\toprule

\textsc{GPT-NER} & 75.44 & 45.74 & 56.95 & 56.83 & 36.2 & 44.23 \\ 
\hspace{0.1cm}+ LLM-verification & - & - & - & - & - & - \\
\hspace{0.1cm}+ LLM-verification \& CoT & - & - & - & - & - & - \\
\hspace{0.1cm}\textbf{+ \textsc{nerve} (Ours)} & \textbf{78.78} & \textbf{50.2} & \textbf{61.32} & \textbf{62.06} & \textbf{41.18} & \textbf{49.5} \\ \midrule

\textsc{ConNER} & 89.48 & 92.22 & 90.83 & 77.07 & 84.53 & 80.63 \\ 
\hspace{0.1cm}+ LLM-verification & - & - & - & - & - & - \\
\hspace{0.1cm}+ LLM-verification \& CoT & - & - & - & - & - & - \\
\hspace{0.1cm}\textbf{+ \textsc{nerve} (Ours)} & 87.9 & 91.62 & 89.72 & 72.49 & 83.79 & 77.73 \\ \midrule

\textsc{BioBERT} & 63.77 & 75.43 & 69.11 & 53.96 & 47.42 & 50.48 \\ 
\hspace{0.1cm}+ LLM-verification & - & - & - & - & - & - \\
\hspace{0.1cm}+ LLM-verification \& CoT & - & - & - & - & - & - \\
\hspace{0.1cm}\textbf{+ \textsc{nerve} (Ours)} & \textbf{70.08} & \textbf{79.25} & \textbf{74.39} & \textbf{62.55} & \textbf{56.68} & \textbf{59.47} \\ 

\bottomrule

\end{tabular}
\caption{Main experimental results of our \textsc{nerve} and compared approaches. Evaluation is done on token-level.}
\label{tab:bio_results}
\end{table*}

==> tables/cross_dataset.tex <==
%수정예정
\begin{table}[h]
% \small
\centering
\resizebox{1.\columnwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
% \multirow{2}{*}{Source $\to$ Target}
{Source $\to$ Target}
 &
  \multicolumn{3}{c}{\textbf{GENIA} $\to$ \textbf{BC5CDR}} &
  \multicolumn{3}{c}{\textbf{BC5CDR} $\to$ \textbf{GENIA}} \\ 
  \cmidrule(lr){2-4} \cmidrule(l){5-7}

  
% \textbf{Models} & 
\textbf{} & 
  P &
  R &
  F &
  P &
  R & 
  F \\ 
\toprule
\textsc{ConNER} (on Target) & 85.67 & 96.47 & 90.75 & 74.13 & 96.69 & 83.92 \\
\hspace{0.1cm}\textbf{+ \verifiner~(Ours)} & - & - & - & 58.15 & 77.42 & 66.42 \\ \midrule

\textsc{BioBERT} (on Target) & 63.87 & 76.06 & 69.44 & 54.51 & 65.30 & 59.42 \\ 
\hspace{0.1cm}\textbf{+ \verifiner~(Ours)} & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{66.49} & \textbf{87.25} & \textbf{75.47} \\ \midrule


\textsc{GPT-NER} (on Target) & 84.69 & 52.98 & 65.19 & 56.44 & 42.15 & 48.26 \\ 

\bottomrule

\end{tabular}}
\caption{Experimental results on unseen settings. Evaluation is done on entity-level.}
\label{tab:cross_dataset_results}
\end{table}

==> tables/goal.tex <==
\begin{table}[h]
\small
\centering
\begin{tabular}{cccc}
\toprule

  \multicolumn{2}{c}{\textbf{BC5CDR}} &
  \multicolumn{2}{c}{\textbf{GENIA}} \\ 
  \cmidrule(lr){1-2} \cmidrule(lr){3-4}
  
% \textbf{Models} & 
  TP to TP &
  FP to TP &
  TP to TP &
  FP to TP \\ 
\toprule
 - & - & - & - \\ 
\bottomrule
\end{tabular}
\caption{Goal Maximization on model-orthogonal benchmark.}
\label{tab:goal}
\end{table}

==> tables/main_table.tex <==
\begin{table*}[!ht]
\small
\centering
 \resizebox{1.\textwidth}{!}{
 
\begin{tabular}{lcccccccccccc}
\toprule
 &
  \multicolumn{6}{c}{\textbf{BC5CDR}} &
  \multicolumn{6}{c}{\textbf{GENIA}} \\ 
  \cmidrule(lr){2-7} \cmidrule(l){8-13}

 &
 \multicolumn{3}{c}{Token-level} &
  \multicolumn{3}{c}{Entity-level} &
  \multicolumn{3}{c}{Token-level} &
  \multicolumn{3}{c}{Entity-level} \\ 
  \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(l){11-13} 
% \textbf{Models} & 
\textbf{} & 
  P &
  R &
  F &
  P &
  R &
  F &
  P &
  R &
  F &
  P &
  R &
  F \\ 
\midrule
% - & - & - &
\textsc{GPT-NER} & - & - & - & 79.84 & \textbf{47.48} & 59.55 & - & - & - & 56.44 & 42.15 & 48.26 \\ 
\hspace{0.1cm}+ Manual Mapping & - & - & - & - & - & - & - & - & - & - & - & - \\
\hspace{0.1cm}+ LLM-verification & - & - & - & 49.94 & 21.37 & 29.93 & - & - & - & 36.52 & 69.53 & 47.89\\
\hspace{0.1cm}+ LLM-verification \& CoT & - & - & - & 49.46 & 20.88 & 29.37 & - & - & - & 22.87 & 48.45 & 31.07\\
\rowcolor{defaultcolor}\hspace{0.1cm}\textbf{+ \verifiner~(Ours)} & - & - & - & \textbf{91.01} & 46.92 & \textbf{61.92} & - & - & - & \textbf{72.37} & \textbf{44.95} & \textbf{55.46} \\ 
\midrule

\textsc{ConNER} & - & - & - & 85.67 & \textbf{96.47} & \textbf{90.75} & - & - & - & 74.13 & \textbf{96.69} & 83.92\\ 
\hspace{0.1cm}+ Manual Mapping & - & - & - & - & - & - & - & - & - & - & - & - \\
\hspace{0.1cm}+ LLM-verification & - & - & - & 48.33 & 27.65 & 35.17 & - & - & - & 47.01 & 99.4 & 63.83 \\
\hspace{0.1cm}+ LLM-verification \& CoT & - & - & - & 53.7 & 31.59 & 39.78 & - & - & - & 30.45 & 85.15 & 44.86 \\
\rowcolor{defaultcolor}\hspace{0.1cm}\textbf{+ \verifiner~(Ours)} & - & - & - & \textbf{87.12} & 88.86 & 87.98 & - & - & - & \textbf{79.07} & 91.82 & \textbf{84.97} \\ \midrule

\textsc{BioBERT} & - & - & - & 63.87 & \textbf{76.06} & 69.44 & - & - & - & 54.51 & 65.30 & 59.42 \\ 
\hspace{0.1cm}+ Manual Mapping & - & - & - & - & - & - & - & - & - & - & - & - \\
\hspace{0.1cm}+ LLM-verification & - & - & - & 29.31 & 22.94 & 25.74 & - & - & - & 35.75 & 85.1 & 50.35 \\
\hspace{0.1cm}+ LLM-verification \& CoT & - & - & - & 36.24 & 28.12 & 31.67 & - & - & - & 23.48 & 66.51 & 34.71 \\
\rowcolor{defaultcolor}\hspace{0.1cm}\textbf{+ \verifiner~(Ours)} & - & - & - & \textbf{83.07} & 71.20 & \textbf{76.68} & - & - & - & \textbf{77.45} & \textbf{67.75} & \textbf{72.31} \\ 

\bottomrule

\end{tabular}}
\caption{Main experimental results of our \verifiner~and compared approaches on token-level and entity-level evaluation.}
\label{tab:main_results}
\end{table*}

==> tables/main_table_old.tex <==
\begin{table*}[ht]
\small
\centering
 \resizebox{1.\textwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
 &
  \multicolumn{3}{c}{\textbf{BC5CDR}} &
  \multicolumn{3}{c}{\textbf{GENIA}} \\ 
  \cmidrule(lr){2-4} \cmidrule(l){5-7}
  
% \textbf{Models} & 
\textbf{} & 
  Precision &
  Recall &
  F1 &
  Precision &
  Recall &
  F1 \\ 
\toprule

\textsc{GPT-NER} & 84.69 & \textbf{52.98} & 65.19 & 56.44 & 42.15 & 48.26 \\ 
\hspace{0.1cm}+ LLM-verification & 49.94 & 21.37 & 29.93 & 36.52 & 69.53 & 47.89\\
\hspace{0.1cm}+ LLM-verification \& CoT & 49.46 & 20.88 & 29.37 & 22.87 & 48.45 & 31.07\\
\hspace{0.1cm}\textbf{+ \nerve~(Ours)} & \textbf{90.53 (\blue{+ 5.84})} & 51.49 (\textcolor{red}{- 1.49}) & \textbf{65.64 (\blue{+ 0.45})} & \textbf{70.85 (\blue{+ 14.41})} & \textbf{45.81 (\blue{+ 3.66})} & \textbf{55.64 (\blue{+ 7.38})} \\ \midrule

\textsc{ConNER} & \textbf{89.32} & \textbf{94.16} & \textbf{91.68} & 77.70 & \textbf{96.54} & 86.10\\ 
\hspace{0.1cm}+ LLM-verification & 48.33 & 27.65 & 35.17 & 47.01 & 99.4 & 63.83 \\
\hspace{0.1cm}+ LLM-verification \& CoT & 53.7 & 31.59 & 39.78 & 30.45 & 85.15 & 44.86 \\
\hspace{0.1cm}\textbf{+ \nerve~(Ours)} & 87.61 (\textcolor{red}{- 1.71}) & 88.23 (\textcolor{red}{- 5.93})& 87.92 (\textcolor{red}{- 3.76}) & \textbf{79.79 (\blue{+ 2.2})} & 94.66 (\textcolor{red}{- 1.88}) & \textbf{86.59 (\blue{+ 0.49})} \\ \midrule

\textsc{BioBERT} & 63.58 & \textbf{75.56} & 69.06 & 54.49 & 63.85 & 58.80 \\ 
\hspace{0.1cm}+ LLM-verification & 29.31 & 22.94 & 25.74 & 35.75 & 85.1 & 50.35 \\
\hspace{0.1cm}+ LLM-verification \& CoT & 36.24 & 28.12 & 31.67 & 23.48 & 66.51 & 34.71 \\
\hspace{0.1cm}\textbf{+ \nerve~(Ours)} & \textbf{81.56 (\blue{+ 17.98})} & 71.74 (\textcolor{red}{- 3.82}) & \textbf{76.34 (\blue{+ 7.28})} & \textbf{77.80 (\blue{+ 23.31})} & \textbf{68.32 (\blue{+ 4.47})} & \textbf{72.75 (\blue{+ 13.95})} \\ 

\bottomrule

\end{tabular}}
\caption{Main experimental results of our \nerve~and compared approaches. Evaluation is done on entity-level.}
\label{tab:main_results}
\end{table*}

==> tables/step2_prompt.tex <==
\begin{table*}
    \small
    \centering
    \begin{tabular}{p{14cm}}
    \toprule
    \textbf{Prompt} \\
    \midrule
    You will be provided with two contradictory persona sentences, along with their source personas and the dialogue fragments from which these persona sentences were derived.

    Your task is to resolve the contradiction between the two persona sentences based on the dialogue fragments and the source persona of each contradictory persona. You can use these two strategies: \\
    \textbf{[Resolution]}: If the two personas are based on the same event but change over time (possibly due to a temporal difference or other events in between), adjust and aggregate them into one new persona sentence. \\
    \textbf{[Disambiguation]}: If the contradiction between them isn’t due to time changes or they are derived from unrelated events in the first place, utilize dialogue fragments to rewrite (clarify/specify) each persona. \\
    First, provide a rationale for your choice ([Resolution] or [Disambiguation]). Then, based on this rationale, generate refined persona sentence(s). 
    
    If the two personas are not contradictory, generate \textbf{[NO\_CONFLICT]}.
    \\ \midrule
    \textcolor{teal}{\textbf{Example 1:}} \\
    \textbf{\texttt{Persona 1}:} I am a programmer. \\
    Dialogue fragment of Persona 1:\\ A: As a computer programmer, I spend a lot of time writing and debugging code. It’s rewarding to see my work contribute to the development of functional and efficient software. \\
    \textit{Source Persona:} I am a programmer. \\
    
    \textbf{\texttt{Persona 2:}} I get fire. \\
    Dialogue fragment of Persona 2:\\ A: I got fired. It was quite unexpected, and I'm still processing everything. \\B: I’m really sorry to hear that. Do you want to talk about what happened? \\
    \textit{Source Persona:} I don't have a job right now. \\
    
    \textbf{\texttt{Rationale:}} There is a temporal connection between the two personas. Persona 1 is about being a programmer, whereas Persona 2 is about having been fired. Both personas can exist over time with Persona 2 occurring after Persona 1. \\
    \textbf{[Resolution]:} I am a programmer who has recently been fired. \\\midrule
    
    \textcolor{teal}{\textbf{Example 2:}} \\
    \textbf{\textit{\texttt{Persona 1}}:} I feel happy. \\
    Dialogue fragment of Persona 1: \\A: My favorite baseball team won this season! I'm so excited! \\B: Wow, really? That's great news! \\
    \textit{Source Persona:} My team won the league. \\
    
    \textbf{\texttt{Persona 2:}} I have been feeling quite stressed. \\
Dialogue fragment of Persona 2: \\A: Work has been overwhelming with tight deadlines and high expectations. It’s been hard to find time for relaxation and self-care. \\B: With stress piling up, it’s important to find ways to unwind and destress. Maybe I’ll try meditation or yoga to help manage my anxiety. \\
    \textit{Source Persona:} I work very hard. \\
    
    \textbf{\texttt{Rationale:}} The two personas do not reflect changes over time but rather different emotional states in response to separate circumstances; one, a moment of happiness due to a favorite team winning, and the other, underlying stress caused by work pressures. \\
    \textbf{[Disambiguation]:} \\
    - \textbf{{\texttt{Persona 1:}}} I feel happy when my favorite baseball team wins. \\
    - \textbf{\texttt{Persona 2:}} I am a person dealing with work-related stress and looking for ways to manage anxiety.\\ \midrule
    \textbf{\textcolor{teal}{\textbf{Example 3:}}} \\
    \textbf{\textit{\texttt{Persona 1}}:} I am a vegetarian. \\
    Dialogue fragment of Persona 1: \\
    A: I’ve been a vegetarian for about 5 years now. It started for health reasons, but now it's also about sustainability and animal welfare. \\
    \textit{Source Persona:} I am a vegetarian. \\
    
    \textbf{\texttt{Persona 2:}} I enjoy reading fiction books. \\
    Dialogue fragments of Persona 2: \\A: One of my favorite pastimes is reading fiction. I love getting lost in different worlds and lives through the pages of a good novel. \\
    \textit{Source Persona:} I enjoy reading fiction books. \\
    
    \textbf{\texttt{Rationale:}} The two persona sentences do not contradict each other as they pertain to different aspects of the speaker’s identity. One persona is about dietary preference (being a vegetarian), and the other is about a hobby or interest (enjoying reading fiction books). There is no inherent conflict between being a vegetarian and enjoying reading fiction, so the two persona sentences can coexist without the need for resolution or disambiguation. \\
    \textbf{[NO\_CONFLICT]} \\ \midrule
    \textcolor{teal}{\textbf{Example 4:}} ... \\ \bottomrule
    \end{tabular}
    \caption{The prompt for \textbf{\textsc{Caffeine}} (Five-shot setting, Examples 4 and 5 are omitted in this table). The ``preservation'' strategy is represented as \textbf{[NO\_CONFLICT]} in our prompt.}
    \label{tab:step2_prompt}
\end{table*}


==> tables/table1.tex <==
\begin{table}[]
\begin{tabular}{ll}
\hline
\multicolumn{1}{c}{\textbf{Method}}  & \multicolumn{1}{c}{\textbf{Acc}} \\ \hline
\textit{w/ description \& examples}  & 33.38                            \\
\textit{w/o description}             & 34.67                            \\
\textit{\textbf{w/o examples}}       & \textbf{33.38}                   \\
\textit{w/o description \& examples} & 11.46                            \\ \hline
\end{tabular}
\end{table}
